Weighted Ensemble Self-Supervised Learning

Ensembling has proven to be a powerful technique for boosting model performance, uncertainty estimation, and robustness in supervised learning. Advances in self-supervised learning (SSL) enable leveraging large unlabeled corpora for state-of-the-art few-shot and supervised learning performance. In this paper, we explore how ensemble methods can improve recent SSL techniques by developing a framework that permits data-dependent weighted cross-entropy losses. We refrain from ensembling the representation backbone; this choice yields an efficient ensemble method that incurs a small training cost and requires no architectural changes or computational overhead to downstream evaluation. The effectiveness of our method is demonstrated with two state-of-the-art SSL methods, DINO (Caron et al., 2021) and MSN (Assran et al., 2022). Our method outperforms both in multiple evaluation metrics on ImageNet-1K, particularly in the few-shot setting. We explore several weighting schemes and find that those which increase the diversity of ensemble heads lead to better downstream evaluation results. Thorough experiments yield improved prior art baselines which our method still surpasses; e.g., our overall improvement with MSN ViT-B/16 is 3.9 p.p. for 1-shot learning.

==> body/background2.tex <==
\newcommand{\dd}{\mathrm d }
\newcommand{\HH}{\operatorname{\mathsf H}}
\newcommand{\KK}{\operatorname{\mathsf K}}
\newcommand{\EE}{\operatorname{\mathsf E}}
\newcommand{\Var}{\operatorname{\mathsf Var}}
\newcommand{\reals}{\mathbb R}
\newcommand{\ints}{\mathbb Z}
\newcommand{\X}{\mathcal X}
\newcommand{\Y}{\mathcal Y}
\newcommand{\Z}{\mathcal Z}
\newcommand{\stopgrad}{\operatorname{stopgrad}}

\clearpage
\section{Background (v2)}\jdnote{TODO: Add citations.}
We first establish notation then introduce our empirically studied SSL methods as maximum likelihood analogues. Denote \href{https://arxiv.org/abs/1406.1385}{unnormalized KL divergence} by $\KK[q(X),p(X)]=\HH^\times[q(X),p(X)]-\HH[q(X)]$ where $\HH[q(X)]=\HH^\times[q(X),q(X)]$, $q,p$ are non-negative integrable functions and,
\begin{align}
\HH^\times[q(X),p(X)]&=-\int_\X q(x)\log p(x) \dd x - \int_\X p(x)\dd x+1
%\\
%\HH[q(X)]&=-\int_\X q(x)\log q(x)\dd x - \int_\X q(x)\dd x+1. && \text{(unnormalized entropy)}
\end{align}
is the unnormalized cross-entropy (where $0\log 0=0)$. 
%These quantities simplify to their usual definitions when $p,q$ are normalized. 

Let $\nu(X, Y)=\nu(X)\nu(Y|X)$ denote nature's distribution of evidence/outcome pairs and let $s(Y|\theta,X)$ be a predictive model of outcomes given evidence parameterized by $\theta \in \mathcal{T}$.
Supervised maximum likelihood seeks the minimum expected conditional population risk wrt $\theta$, 
\begin{align}
\EE_{\nu(X)}\KK[\nu(Y|X),s(Y|\theta,X)] = \EE_{\nu(X)}\HH^\times[\nu(Y|X),s(Y|\theta,X)]-\EE_{\nu(X)}\HH[\nu(Y|X)].
\end{align}

We henceforth omit $\EE_{\nu(X)}\HH[\nu(Y|X)]$ since it is constant in $\theta.$ Since $\nu(X, Y)$ is unknown, a finite sample approximation is often employed. Denoting a size-$n$ iid training set by  $\mathcal{D}_n=\{x_i\}_i^n\sim\nu^{\otimes n}$ and empirical distribution by $\hat \nu(X, Y)=\frac{1}{n}\sum_{x\in\mathcal{D}_n,y\sim\nu(Y|x)}\delta(X-x)\delta(Y-y),$ the sample risk is characterized by
%\begin{align}
$-\tfrac{1}{n} \sum_{x\in\mathcal{D}_n}\HH^\times[\hat\nu(Y|x),s(Y|\theta,x)].$
%\end{align}

In self-supervised learning (SSL), we further assume $\hat\nu(Y|X)$ is inaccessible and/or unreliable. Under this modification, some SSL techniques adapt the above framework by substituting $\hat\nu(Y|X)$ for a weakly learned target or ``teacher'', $t(Y|x).$ The loss becomes
%\begin{align}
$-\tfrac{1}{n} \sum_{x\in\mathcal{D}_n}\HH^\times[t(Y|x),s(Y|\theta,x)].$
%\end{align}

In DINO, MSN, and our experiments, the student model is defined as,
\begin{align}
s(Y|\theta,x) &= \softmax\left(\left\{\frac{1}{\tau}\frac{(h_\psi\circ f_\omega)(x)\cdot \mu_y}{\|(h_\psi\circ f_\omega)(x)\|_2\|\mu_y\|_2}:y\in[k]\right\}\right)\\
\theta&=\{\psi,\omega,\{\mu_y\}_{y\in[k]}\}\in\mathcal{T},
\end{align}
where $f_\omega:\X\to\Z$ is the backbone model, $h_\psi:\Z \to \reals^d$ is the head model, and $\mu_y\in\reals^d$ is a global representation (i.e., ``centroid''). Hyperparameters $\tau,k$ control temperature and the number of centroids. The teacher is defined as $t(Y|x) = s(Y|\stopgrad(g(\theta)),x)$ where $g:\mathcal{T}\to\mathcal{T}$ is an exponential moving average of gradient descent iterates.

To prevent degeneracy in the above loss, regularization such as Sinkhorn normalization or mean-entropy regularization are essential. For brevity we omit these details from our exposition.


==> body/background_saurabh.tex <==
%\clearpage
\section{Background}
\label{sec:background}

In this section, we review recent SSL methods from the perspective of maximum likelihood estimation (MLE), with an emphasis on self-distillation approaches used in our experiments.
This MLE formulation provides a tool for establishing our framework for ensemble losses in \cref{sec:method}.

%\aanote{I think the background is a good place to layout the motivation of the paper.  I'd suggest opening the background with the sort of central story of the of the paper.  SSL techniques are hot right now and ensembling works for other areas so here we set out to try to see if we could show benefit to SSL techniques with ensembling.  However, as soon as you decide to do that you realize that there is a lot of different ways that could be accomplished.  In particular, we first need to describe in better details how some of the existing SSL techniques currently work... (that motivates why we need some background on SSL techniques and also hooks the reader for why they should also care and signals to them what they should pay particular attention to in the review)}

\paragraph{From Maximum Likelihood to SSL}
\yrnote{I feel it is better to have this section relating SSL with MLE and introducing the teacher/student, insetad of purely introducing maximum likelihood}
We first establish notations then introduce our empirically studied SSL methods as maximum likelihood analogues. Denote unnormalized KL divergence \citep{dikmen2014learning} by $\KK[p(X),q(X)]=\HH^\times[p(X),q(X)]-\HH[p(X)]$ where $\HH[p(X)]=\HH^\times[p(X),p(X)]$, $p,q$ are non-negative integrable functions and, $\HH^\times[p(X),q(X)]&=-\int_\X p(x)\log q(x) \dd x + \int_\X q(x)\dd x-1$ is the unnormalized cross-entropy (where $0\log 0=0)$. 
% \yrnote{we need to motivate why we use unnormalized CE/KL.}
These quantities simplify to their usual definitions when $p,q$ are normalized, but critically they permit us to show that unnormalized weighting factors for the distributions in MLE setting are still a principled choice.

Let $\nu(X, Y)=\nu(X)\nu(Y|X)$ denote nature's distribution of
\yrnote{can we rename evidence/outcome to input/label of input/target which may be more natural to ML audience?}
evidence/outcome pairs over the space $\X\times \Y$ and let $s(Y|\theta,X)$ be a predictive model of outcomes given evidence parameterized by $\theta \in \mathcal{T}$.
Supervised maximum likelihood seeks the minimum expected conditional population risk with respect to $\theta$, 
\begin{align}
\arg\min_{\theta} \EE_{\nu(X)}\KK[\nu(Y|X),s(Y|\theta,X)] =
\arg\min_{\theta}  \EE_{\nu(X)}\HH^\times[\nu(Y|X),s(Y|\theta,X)]+\text{constant}
\end{align}

Since $\nu(X, Y)$ is unknown, a finite sample approximation is often employed. Let $\hat \nu(X, Y)$ be the empirical distribution, then sample risk is characterized by
%\begin{align}
$-\tfrac{1}{n} \sum_{x\in\mathcal{D}_n}\HH^\times[\hat\nu(Y|x),s(Y|\theta,x)].$
%\end{align}
Write the Kronecker delta function $\delta:\reals\to\{0,1\}$ as $1$ when $x=0$ and $0$ otherwise. Denote a size-$n$ \iid training set by  $\mathcal{D}_n=\{x_i, y_i\}_i^n\sim\nu^{\otimes n}$ and empirical distribution by $\hat \nu(X, Y)=\frac{1}{n}\sum_{x\in\mathcal{D}_n,y\sim\nu(Y|x)}\delta(X-x)\delta(Y-y).$

\yrnote{I would not write out the empirical risk, and just briefly mention it for simplicity, and introduce delta function later when needed.}
\iansf{This paragraph should start outlining how we go from the empirical distribution to the teacher, I think.}

\yrnote{I would consider instead call this self-distillation, if teacher/student is moved to the previous part.}
\jdnote{Assuming I understand, I agree about renaming this subsection to "Self-Distillation".}
In SSL setup, we further assume $\hat\nu(Y|X)$ is inaccessible and/or unreliable. 
Under this modification, some SSL techniques adapt the above framework by substituting $\hat\nu(Y|X)$ for a weakly learned target or ``teacher'', $t(Y|x).$ 
\yrnote{I would explain that ``SSL methods use a surrogate task'' denoted by \eg, $K$ to make clear the difference. And then say ``in self-distillation methods, it is induced by a learned codebook''}
\yrnote{I would also add data augmentation to the loss because it is key to SSL. We may say that `typically differently augmented data from the same input is used for the student and teacher for learning the augmentation invariance.'}
The loss becomes
%\begin{align}
$-\tfrac{1}{n} \sum_{x\in\mathcal{D}_n}\HH^\times[t(Y|x),s(Y|\theta,x)].$
%\end{align}

\paragraph{Teacher and student in codebook SSL methods}
For self-distillation methods, \eg, DINO \citep{caron2021dino}, MSN \citep{assran2022msn}, the student model predicts its `code' over a learnable codebook,
\begin{align}
s(Y|\theta,x) &= \softmax\left(\left\{\frac{1}{\tau}\frac{(h_\psi\circ r_\omega)(x)\cdot \mu_y}{\|(h_\psi\circ r_\omega)(x)\|_2\|\mu_y\|_2}:y\in[c]\right\}\right)\label{eq:student}\\
\theta&=\{\psi,\omega,\{\mu_y\}_{y\in[c]}\}\in\mathcal{T},\label{eq:params}
\end{align}
\yrnote{I made $\mathcal{Z}$ explicit to $\reals^l$ for consistency. }
where $r_\omega:\X\to\Z$ is the encoder that outputs the representations for downstream tasks, $h_\psi:\Z \to \reals^d$ is the projection head, and $\mu_y\in\reals^d$ is a codebook entry (\ie, a ``centroid'').
% a global representation (i.e., a ``centroid'' or a codebook entry).
\cref{eq:student} can be viewed as ``soft clustering'' \citep{caron2020swav}, where the input is assigned to those centroids that are closer to the projection head's output.
% is to assign higher probabilities to those centroids, $\{\mu_y\}_{y\in[c]}$, which are closer to the projection head's output. (in cosine similarity).
\yrnote{edited the previous two sentences}
Although the distinction between encoder and projection head is arbitrary, it is empirically found to be important for representation performance on downstream tasks \citep{chen2020simclr,chen2020simclrv2}, where the head and codebook are discarded.
Hyperparameters $\tau\in\reals_{>0},c\in\ints_{>0}$ represent temperature and the number of centroids.
The teacher is defined as $t(Y|x) = s(Y|\stopgrad(g(\theta)),x)$ where $g:\mathcal{T}\to\mathcal{T}$.
\yrnote{I'd like to suggest that we still use $\bar{\theta}$ to make it more clear it is another $\theta$.}
Commonly, $g(\theta)$ is an exponential moving average of gradient descent iterates.
\yrnote{we may want to mention that the temperature for the student and teacher is different to make it more clear, and also consistent with notations in the later parts.}

To prevent degeneracy and capture desired invariances, strong data augmentation 
\yrnote{I think data augmentation needs to be explicit, it is not only for preventing degeneracy but also for learning invariance.}
and techniques for avoiding representation collapse (\eg, Sinkhorn-Knopp normalization in \citet{caron2020swav}, mean entropy maximization regularization \citet{assran2022msn} \etc) are essential. Although critical to SSL effectiveness, they are not relevant to our proposed methods and omitted for brevity.



==> body/method1.tex <==

%$\enttemp$ is the hyper-parameter that controls the temperature of entropy weighting.
%This loss has several interesting properties:
%First, it generalizes the `\outside' \sinote{consider removing the single quotes here and elsewhere that strategies are used, and use a different font instead}
%\yrnote{good idea, will do!}
%\yrnote{I may overly use this abbreviation.}
%strategy (the special case when $\enttemp=\infty$) by introducing an importance weight as with `\outside'. 
%Second, the importance weights $\weight_j$ are explicitly introduced and are inversely correlated with the entropy of teacher predictions.
%In other words, the head whose teacher has a lower entropy (\ie, higher confidence about its prediction) is given larger importance weights for learning the representations, which also aligns with the rule of thumb in \citet{wang2022asym}.\aanote{remind the reader what the rule of thumb in Wang was}
%\yrnote{is the last statement accurate? I'm putting this because for Gaussian distribution (though it's not), the variance is directly related with the entropy. Or do we need to explain more?}
% An alternative is to weight by the entropy of student predictions of each head instead, 
%Third, the entropy weighting is data-dependent, \ie, conditioned on the input, different heads can be the dominant (\ie, most confident) one. 
%This potentially causes different heads to \emph{specialize} in different data regions, similar to the mixture of expert model \citep{jacobs1991moe}.
%Finally, unlike the `\inside' strategy, interaction between different heads is minimally introduced only through the weight computation, which may further encourage the diversity.


%\rule{\textwidth}{1pt}
%\clearpage




\aanote{I'd suggest adding little code snippets for each of the ensembling methods, with these kinds of things a lot of time the mathematical notiation is more confusing than a little code snipper, and the code snippet is unambiguous.}
\input{body/pseudo_code_ens_loss}
\yrnote{added code for computing the loss, the full code in \cref{appx:pseudo_code}. I guess probably we won't include this in the main body, because I feel it does not provide a lot but takes a lot of space. A good figure should be more helpful.}

Given an ensemble of predictive distributions $\set{\sdist^{j}(K^{j} \cond \sinp), \tdist^{j}(K^{j} \cond \tinp)}_{j \in [\numens]}$, the question is how to train them.
Here we explore different design choices.
Our key insight is that \emph{gradient importance weights} need to be introduced (implicitly or explicitly) to encourage the diversity across ensemble heads.

\yrnote{would like to see some suggestions about paragraph titles}
% \paragraph{Outside-log average}
\paragraph{Uniform weighting (\outside)}
This simplest approach is to treat different heads as independent and directly average the cross-entropy loss over them, \ie,
\begin{align}
    \lossout = \frac{1}{\numens} \sum_{j \in [\numens]} \CE{\tdist^{j}(K^{j} \cond \tinp)}{\sdist^{j}(K^{j} \cond \sinp)}
\end{align}
% over ensembles and we call it the `\outside' strategy because the average over ensembles is outside the logarithm of loss computation.
This strategy introduces \textit{uniform} weights $\weight_j = \frac 1 \numens$ over ensemble elements.
% , thus we name it the `\outside' strategy.
Though plausible, we empirically find that this strategy leads to no gain over a single head.
In particular, different heads tend to learn the same semantic mappings even when randomly initialized; \ie, the code assignments in different heads become homogeneous up to permutation.
See \cref{fig:vis_ens_head_diversity} for a visualization.
\aanote{I think this strategy should be compared to a single head with a larger codebook, as it seems like it would be most similar to that.}

% \paragraph{Inside-log average}
\paragraph{Probability weighting (\inside)}
An alternative is to first average the predictive distributions and then compute the cross-entropy loss, \ie,
\begin{align}
    \lossin = \CE{\frac{1}{\numens} \sum_{j \in [\numens]} \tdist^{j}(K^{j} \cond \tinp)}{\frac{1}{\numens} \sum_{j \in [\numens]} \sdist^{j}(K^{j} \cond \sinp)}
\end{align}
There are some interesting facts about this strategy: 
First, averaging the predictive distributions introduces correspondence between codes from different heads (\ie, $K^j$),
\yrnote{is using $K^j$ accurate? please double check this statement, I'm not sure if it is the case anymore because I realize it might contradict the visualization in \cref{fig:vis_ens_head_diversity}}
thus different heads are are no longer independent but `coorperative' for solving the same SSL task.
Second, the mean teacher prediction $\meantdist =  \sum_{j \in [\numens]} \frac{\tdist^j}{\numens}$ \iansf{Missing some words here.} as the surrogate target distribution, which reduces the variance of teacher predictions.
This aligns with the rule of thumb studied by \citet{wang2022asym} that a lower-variance teacher benefits Siamese representation learning.
Third, $\lossin$ lower bounds $\lossout$ up to a constant due to the joint convexity of KL divergence and the fact that teacher predictions $\tdist^j$ are fixed.
\yrnote{We may not include this because 1) the paragraph might be too long for a main method; 2) not sure if this lower bound is interesting}
Finally, this loss implicitly introduces importance weights for gradients with respect to different heads, similar to importance-weighted autoencoder \citep{burda2015iwae}:\aanote{I don't understand this.}
\begin{align}
    \nabla \lossin 
    &= - \nabla \sum_{k \in [\numcode]}  \meantdist(k \cond \tinp) \log \pa{\frac{1}{\numens} \sum_{j \in [\numens]} \sdist^{j}(k \cond \sinp)} \\
    &= - \sum_{j \in [\numens]} \sum_{k \in [\numcode]}  \weight_{jk} \cdot \meantdist(k \cond \tinp) \nabla \log\pa{\sdist^{j}(k \cond \sinp)}
\end{align}
where $\weight_{jk}= \sdist^{j}(k \cond \sinp) / \sum_{j \in [\numens]} \sdist^{j}(k \cond \sinp)$ are the normalized importance weights based on student predicted probabilities.
For each code $k$, the head $j$ that predicts with larger probability receives larger weights, causing each head to `specialize' on different codes for different inputs.
\yrnote{this statement may not be true. Any suggestions?}
This can be viewed as a soft version of multiple choice learning \citep{guzman2012mcl} used in multi-headed networks \citep{lee2015multihead}, which (if reinterpreted in our setting) sets an explicit weight only to the head with maximum predicted probability, \ie, $\weight_{jk} = \ind{j = \argmax_{i \in \numens} \weight_{ik}}$ ($\argmax$ breaks ties arbitrarily).
We empirically find this strategy leads to more diverse heads and improved performance over `\outside'.

(Only need to study the gradient. Looking at the gradient, we see that it is importance weighting based on relative probability among the teachers. The more one-hot the teacher is, the lower its entropy is, which leads to directly studying negative entropy weighting below.)

\tofill{}
This strategy can be generalized by explicitly introducing the importance weights with temperature or weighting by the teacher model.

\tofill{} Main points: 
Treating different projection head to operate in the same space. Lower variance teacher, weighted by student confidence. 
Empirically better than naive outside average. Analysis of gradient with importance weight. Similarity to IWAE. Bound on the outside average.
Probably try argmax or weighted by teacher.

% \paragraph{Entropy-weighted average} 
\paragraph{Entropy weighting (\ew)} 
Though the `\inside' strategy increases the ensemble head diversity with implicit gradient weighting, it may not fully exploit the advantage of ensembling as it may overly introduce correlation between heads by directly averaging over heads.
\yrnote{this statement could be much improved.}
Motivated by this, we seek a strategy that makes different heads operate more independently (as with `\outside') and introduces importance weighting to encourage diversity.
We propose the following loss that explicitly introduces a weight for each head based on the \emph{entropy of teacher predictions}:
\begin{align}
    \lossew &= \sum_{j \in [\numens]} \weight_j \CE{\tdist^{j}(K^{j} \cond \tinp)}{\sdist^{j}(K^{j} \cond \sinp)} \\
    \text{where,} \quad  \weight_j &=  \frac{\exp\pa{-\H{\tdist^{j}(K^{j} \cond \tinp)} / \enttemp}}{\sum_{i \in [\numens]} \exp\pa{-\H{\tdist^{i}(K^{i} \cond \tinp)} / \enttemp}}
\end{align}
$\enttemp$ is the hyper-parameter that controls the temperature of entropy weighting.
This loss has several interesting properties:
First, it generalizes the `\outside' \sinote{consider removing the single quotes here and elsewhere that strategies are used, and use a different font instead}
\yrnote{good idea, will do!}
\yrnote{I may overly use this abbreviation.}
strategy (the special case when $\enttemp=\infty$) by introducing an importance weight as with `\outside'. 
Second, the importance weights $\weight_j$ are explicitly introduced and are inversely correlated with the entropy of teacher predictions.
In other words, the head whose teacher has a lower entropy (\ie, higher confidence about its prediction) is given larger importance weights for learning the representations, which also aligns with the rule of thumb in \citet{wang2022asym}.\aanote{remind the reader what the rule of thumb in Wang was}
\yrnote{is the last statement accurate? I'm putting this because for Gaussian distribution (though it's not), the variance is directly related with the entropy. Or do we need to explain more?}
% An alternative is to weight by the entropy of student predictions of each head instead, 
Third, the entropy weighting is data-dependent, \ie, conditioned on the input, different heads can be the dominant (\ie, most confident) one. 
This potentially causes different heads to \emph{specialize} in different data regions, similar to the mixture of expert model \citep{jacobs1991moe}.
Finally, unlike the `\inside' strategy, interaction between different heads is minimally introduced only through the weight computation, which may further encourage the diversity.



% \newcommand{\K}{\operatorname{\mathsf{K}}}
% \renewcommand{\H}{\operatorname{\mathsf{H}}}
% \renewcommand{\E}{\operatorname{\mathsf{E}}}
% \newcommand{\iidm}{\stackrel{\tiny{\mathrm{iid}}}{\sim}}
% \newcommand{\reals}{\mathbb{R}}

% For ensembles....

% %\begin{align}
% %t_{\bar\theta}(K|x^{(t)}) &=  \frac{1}{m'}\frac{1}{m''}\sum_{j\in[m']}\sum_{j'\in[m'']}\softmax\left(\frac{1}{\tau^{(t)}}\frac{r_j^{(t)}\cdot \bar\mu_{j'}}{\|r_j^{(t)}\cdot  \bar\mu_{j'}\|_2} \right)\\
% %t_{\bar\theta}(K|x^{(t)}) &=  \softmax\left(\frac{1}{m'}\frac{1}{m''}\sum_{j\in[m']}\sum_{j'\in[m'']}\frac{1}{\tau^{(t)}}\frac{r_j^{(t)}\cdot \bar\mu_{j'}}{\|r_j^{(t)}\cdot  \bar\mu_{j'}\|_2} \right)
% %\end{align}

% todo:yangjun: change z to r


% \begin{align}
% \mathrm{a}.&\quad \K\left[
%   \tfrac{1}{m}\sum_j^{m} t_{\bar\theta,j}(K|z_{i,j}),
%   \tfrac{1}{m'}\sum_{j'}^{m'} s_{\theta,j'}(K|\tilde{z}_{i,j'})
% \right]
%  && \text{(KL-avg)}\\
% \mathrm{b}.&\quad \cancel{\tfrac{1}{m'}\sum_{j'}^{m'} \K\left[
%   \tfrac{1}{m}\sum_j^{m} t_{\bar\theta,j}(K|z_{i,j}),
%   s_{\theta,j'}(K|\tilde{z}_{i,j'})
% \right]}
%  && \text{(same as $``$e" if $\bar\theta$ is stopped)}\\
% \mathrm{c}.&\quad \cancel{\tfrac{1}{m}\sum_j^{m} \K\left[
%   t_{\bar\theta,j}(K|z_{i,j}),
%   \tfrac{1}{m'}\sum_{j'}^{m'} s_{\theta,j'}(K|\tilde{z}_{i,j'})
% \right]}
%  && \text{(same as $``$a" if $\bar\theta$ is stopped)}\\
% \mathrm{d}.&\quad \tfrac{1}{m}\sum_j^{m} \K\left[
%   t_{\bar\theta,j}(K|z_{i,j}),
%   s_{\theta,j}(K|\tilde{z}_{i,j})
% \right]
%  && \text{(avg-KL)}\\
% \mathrm{e}.&\quad \tfrac{1}{mm'}\sum_j^{m} \sum_{j'}^{m'} \K\left[
%     t_{\bar\theta,j}(K|z_{i,j}),
%     s_{\theta,j'}(K|\tilde{z}_{i,j'})
% \right]
%  && \text{(all-pairs-avg-KL)}\\
% \end{align}

% where (eg)

% \begin{align}
% t_{\bar\theta,j}(K|x^{(t)}) &=  \softmax\left(\frac{1}{\tau^{(t)}}\frac{r_j^{(t)}\cdot \bar\mu_j}{\|r_j^{(t)}\cdot  \bar\mu_j\|_2} \right)\\
% \end{align}

% where \emph{either} $\bar\mu_j = \bar\mu_i$ or $r_j=r_i$ or both or neither.

==> body/method2.tex <==

% Siamese SSL losses are degenerate because the student is trying to match the teacher and the teacher is itself learned.  Our insight is to replicate students and teachers and weight different pairs thereof differently, under some reflection of our belief in the reasonableness of that pair on a particular datum.

% The data-dependent weighting function allows us to capture our intuitions about when we can trust a particular teacher, based on properties of each teacher independently or the group of teachers collectively.

% Before we dive in to our idea we'd like to first frame existing SSL ideas as being a weak form of maximum likelihood. We do this because there is no reason to believe the siamese SSL techniques will result in nondegenerate hypotheses and therefore weighting an ensemble of these (possibly degenerate losses) also inherits these concerns. Nevertheless we found it useful to intuit siamese SSL in this light and that inspired us to weight different teachers differently because there's no real reason to believe in any of the teachers. Put differently: we have no faith in any teacher but relatively speaking we like some teachers more than others wrt a specific datum.

\section{Method (v2)}
% \jdnote{Context: Yangjun asked me to write a "Methods v2" section which I did with the help of Saurabh and Warren.}



In this work we generalize the above framework by using a weighted ensemble model. I.e.,
\begin{align}
\tfrac{1}{n}\sum_{x\in\mathcal{D}_n}\sum_{i,j\in[m]}\HH^\times[w_{ijY}(\theta,x)\odot t_i(Y|x),s(Y|\theta_j,x)] \label{eq:ensemble_loss}
\end{align}

where $\{t_i\}_{i \in [m]}$ and $\{s_j\}_{j \in [m]}$ are collections of teachers and students and,
\begin{align}
w_{ijy}
&=\softmax\left(\left\{\tfrac{1}{\gamma}f_{ijy}(\stopgrad(\theta),x) :i,j\in[m]\right\}\right)\label{eq:ensemble_weight}\\
\theta &\in \{((\psi_j,\omega_j,\{\mu_{jy}\}_{y\in[c]}):j\in[m])\in\mathcal{T}^m:\omega_i=\omega_j\} \label{eq:ensemble_params}.
\end{align}

This generalization enables learning different representations by facilitating ensemble member specialization as dictated by $w_{ijy}$, a function of teacher, student, outcome, and evidence. Equation \eqref{eq:ensemble_loss} uses unnormalized cross-entropy thus enabling a richer class of weights, i.e., $\int_\Y w_{ijy}(\theta,x) t_i(y|x) \dd y$ need not be one.
The ensemble parameter space \eqref{eq:ensemble_params}, implies backbone, head, and cluster architectures are identical among all ensemble members and also indicates that the backbone parameters are not ensembled.

The term $f_{ijk}$ is a diffeomorphic characterization of the weights. As shown in the experiments section, the best performing choice was $f_{i}=-\HH[t_i(Y|x)],$ i.e., low entropy teachers dominate the loss and independently from the student ensemble.

The generality of the above framework enables an infinite number of weighting schemes; we studied:

\begin{align}
%f_{ijy} &=\log \delta(i-1)+\log\delta(j-1)     && \text{(Non-Ensemble)}\\
f_{ijy} &=0                                    && \text{(Favors all equally)}\\
f_{ijy} &= \log s(y|\theta_j,x)                && \text{(Favors opinionated student)}\\
f_{ijy} &= \log t_i(y|x)                       && \text{(Favors opinionated teachers)}\\
f_{ijy} &= -\HH[t_i(Y|x)]                      && \text{(Favors low entropy teachers)}\\
f_{ijy} &= -\HH[s(Y|\theta_j,x)].              && \text{(Favors low entropy students)}
\end{align}

(These correspond to stronger reductions of the entropy of the teacher or the student...)

It is impossible to fully explore the space of weightings; the following might also have been interesting to study,
\begin{align}
f_{ijy} &= -\KK[t_i(Y|x),s(Y|\theta_j,x)]        && \text{(Favors disagreeing teacher/student pairs)}\\
%f_{ijy} &= -\KK[s(Y|\theta_j,x),t_i(Y|x)]       && \text{(KL Student)}\\
f_{ijy} &= -\tfrac{1}{2}\log(c+\Var_{s(Y|\theta_j,x)}[Y]) && \text{(Favors low variance students; e.g., $c=\tfrac{1}{12}$)}\\
f_{ijy} &= -\tfrac{1}{2}\log(c+\Var_{t_i(Y|x)}[Y]).  && \text{(Favors low variance teachers)}
\end{align}

Note that all of the above importance scores can be restricted to one-to-one teacher/student pairs by the modification, $f_{ijy}+\log\delta(i-j)$ where $\delta(x) = \begin{cases}1 & x=0 \\ 0 & x\ne 0\end{cases}$ denotes the Kronecker delta function. Observe that when $f_{ijy}$ is constant in $y$, the normalized definition of cross-entropy is equivalent to the above formulation. In Appendix XXX we offer additional analysis which shows the relationship between some of the proposed weighting schemes.

Recall that we limited our framework to identical backbone parameters $\omega$. This was to ensure that the downstream task's computational cost is unchanged.
Also, by parameterizing via identical replication,  $\mathcal{T}^m$, we artificially limit our  study to homogeneous architectures. Relaxing these assumptions is left as an interesting topic for future study.

While our notational framing was clearly tailored for DINO, MSN type methods, it is likely applicable for a broader class of methods, especially those which use a head/backbone model.
%For example, we can recover the swapping aspect of SWaV, i.e., the  $f_{ijy}=\log\left(1+\frac{\nabla_\theta [s(y|\theta_j,x)\log t_i(y|x)]}{\nabla_\theta [t_i(y|x)\log s(y|\theta_j,x)]}\right) + \log\delta(i-j)$ roughly recovers SWaV, up to a $x$ specific normalizing weight.

\begin{figure}[ht!]
\input{body/approach_fig}
\caption{This is a caption.}
\end{figure}

\aanote{Given constraints on space, I'd move this section to an appendix but pay service to it in the main body.  Highlight that we spent time thinking about just how vast the space of possible ensembling methods is and can think about that space as choosing a single three component weight tensor.  Invite readers to check out the appendix for some further inspiration for future work.}


==> body/method_unified.tex <==
\section{Background and Methods}

Ensembling SSL can mean many things.
We focus on a small subset of the possible space, but we also give a general framework for studying the space.
The framework provides a mathematical intuition pump for generating alternative data-dependent weightings of the cross entropy loss.
We provide the mathematical details in the appendix.
Here, we give a simpler description of the particular ensemble SSL losses we empirically study in this paper.

What did we do?

What is the intuition behind each choice?

What does the framework provide?
\begin{itemize}
\item General non-negative weighting of ensemble entropy terms.
\item Support for the full $n^2$ interactions between ensemble members (as in Prob weighting example).
\item Weights can be unrestricted real functions of the data and the model parameters.
\item Constraints on the weight functions to prevent complex gradient feedback to the model parameters through the weight function.
\end{itemize}

==> body/pseudo_code_ens_loss.tex <==
\begin{minipage}{.68\linewidth}
\begin{algorithm}[H]
\tiny
\SetAlgoLined
    \PyComment{b, n, c,: batch size, number of ensemble heads, codebook size} \\
    \PyComment{log\_ps, log\_pt: student, teacher log probabilities with n ensembles}\\
    \PyComment{strategy: ensemble loss average strategy} \\
    \PyComment{tau\_ent: temperature for entropy weighting}\\
    ~\\
    \PyCode{def ensemble\_loss(log\_ps, log\_pt, strategy, tau\_ent):}\\
    \Indp
        \PyCode{b, n, c = log\_pt.shape} \PyComment{axis 1 corresponds to ensemble} \\
        \PyCode{log\_pt = stop\_grad(log\_pt)} \PyComment{stop gradient for teacher}\\
        ~\\
        \PyCode{if strategy == "Unif":}\\
        \Indp
            \PyCode{loss = - (exp(log\_pt) * log\_ps).sum(axis=-1)} \\
            \PyCode{loss = loss.mean(axis=1)} \PyComment{average over ensembles}\\
        \Indm
        \PyCode{elif strategy == "Prob":}\\
        \Indp
            \PyCode{log\_mean\_pt = logsumexp(log\_pt, axis=1, b=1/n)} \PyComment{mean teacher}\\
            \PyCode{log\_mean\_ps = logsumexp(log\_ps, axis=1, b=1/n)} \PyComment{mean student}\\
            \PyCode{loss = - (exp(log\_mean\_pt) * log\_mean\_ps).sum(axis=-1)} \\
        \Indm
        \PyCode{elif strategy == "Ent":}\\
        \Indp
            \PyCode{ent = - (exp(log\_pt) * log\_pt).sum(axis=-1)} \PyComment{teacher entropy} \\
            \PyCode{weight = softmax(-ent/tau\_ent, axis=1)} \PyComment{entropy weights}\\
            \PyCode{loss = - (exp(log\_pt) * log\_ps).sum(axis=-1)} \\
            \PyCode{loss = (loss * weight).sum(axis=1)} \PyComment{entropy weighted average}\\
        \Indm
        ~\\
        \PyCode{return loss.mean()} \PyComment{average over samples} \\
    \Indm
\caption{Pseudocode for computing ensemble loss}
\label{alg:ensemble_loss}
\end{algorithm}
\end{minipage}


==> figures/plots/tikz_plot_example.tex <==
%%%%tikz
\definecolor{sns1}{rgb}{0.86, 0.3712, 0.33999999999999997}
\definecolor{sns2}{rgb}{0.7247999999999999, 0.86, 0.33999999999999997}
\definecolor{sns3}{rgb}{0.33999999999999997, 0.86, 0.5792000000000002}
\definecolor{sns4}{rgb}{0.33999999999999997, 0.5167999999999995, 0.86}
\definecolor{sns5}{rgb}{0.7871999999999999, 0.33999999999999997, 0.86}

\usepackage{tikz}
\usetikzlibrary{backgrounds, calc, chains, fit, matrix, positioning, shadows, shapes, circuits.ee}
\tikzset{input/.style={}}
\tikzset{output/.style={}}
\tikzset{op/.style={circle, draw, thick, fill=black!10, minimum size=2.5ex, inner sep=0.1ex}}
\tikzset{filter/.style={rectangle, draw, thick, fill=black!10, minimum size=3.5ex, inner sep=1ex}}
\tikzset{other/.style={rounded rectangle, draw, fill=white, minimum size=3.5ex, inner xsep=1ex}}
\tikzset{nn/.style={trapezium, trapezium angle=80, draw, thick, fill=black!10, inner sep=1ex}}
\tikzset{branch/.style={circle, draw, thick, fill=black, minimum size=.5ex, inner sep=0ex}}
\tikzset{tensor/.style={rectangle, draw, thick, fill=white, minimum size=2em, double copy shadow={shadow xshift=.5ex,shadow yshift=-.5ex}}}
\tikzset{image/.style={rectangle, draw, thick, fill=white, minimum size=2em}}
\tikzset{block/.style={rectangle, draw, fill=white, minimum size=2em}}
\tikzset{>=direction ee}

\usepackage{pgfplots}
\pgfplotsset{compat=1.14}
\pgfplotsset{every axis/.append style={enlargelimits={abs=3pt},grid,axis lines=left}}
\pgfplotsset{every axis plot/.append style={thick,mark size=1.5pt,line join=bevel,mark options={solid}}}
\pgfplotsset{label style={font=\small}}
\pgfplotsset{tick label style={font=\footnotesize}}
\pgfplotsset{grid style={color=black!10}}
\pgfplotsset{legend style={draw=none,opacity=.85,font=\footnotesize,cells={anchor=west,opacity=1}}}
\pgfplotsset{every non boxed x axis/.style={xtick align=center,shorten <=-.5\pgflinewidth}}
\pgfplotsset{every non boxed y axis/.style={ytick align=center,shorten <=-.5\pgflinewidth}}
\pgfplotsset{every non boxed z axis/.style={ztick align=center,shorten <=-.5\pgflinewidth}}
\pgfplotsset{/pgf/number format/1000 sep={\,}}

\begin{tikzpicture}
    \begin{semilogxaxis}[
        height=5cm,
        width=8.88cm,
        grid=major,
        log basis x=10,
        xmin=0.01,
        xmax=1.0,
        ymin=32,
        ymax=53,
        xlabel={Relative Compression Ratio},
        ylabel={Classification Error},
        legend style={at={(0.66,0.9)},anchor=north west}
    ]
        
    \addplot[color=sns5,mark=star, mark size=4pt,line width=2pt,dashed] coordinates {
        (1.000000, 33.390000)
    };
    \addlegendentry{Lossless}
    \addplot[color=sns4,mark=diamond*, mark size=5pt,line width=1pt,dashed]  coordinates {
        (0.603237, 33.410000)
    };
    \addlegendentry{16 Bit Gzip}
    \addplot[color=sns3,mark=*, mark size=2pt,line width=1pt,dashed] coordinates {
        (0.610654, 33.390000)
        (0.284684, 33.430000)
        (0.204900, 33.550000)
        (0.099563, 35.710000)
        (0.030696, 89.290000)
        (0.029655, 99.000000)
    };
    \addlegendentry{Quantized}
    \addplot[color=sns2,mark=*, mark size=2pt,line width=1pt,dashed] coordinates {
        (0.000552, 98.300000)
        (0.001103, 96.880000)
        (0.002207, 92.600000)
        (0.004414, 83.540000)
        (0.008828, 68.720000)
        (0.017655, 50.710000)
        (0.035311, 40.080000)
        (0.070621, 36.390000)
        (0.141243, 34.010000)
        (0.282486, 33.570000)
    };
    \addlegendentry{PCA}
    \addplot[color=sns1,mark=*, mark size=2pt,line width=1pt] coordinates {
        (0.013999, 44.662001)
        (0.025043, 37.053999)
        (0.033298, 36.590002)
        (0.054865, 34.374001)
        (0.090031, 34.157999)
        (0.134282, 33.029997)
        (0.166094, 33.622000)
        (0.188537, 33.893998)
        (0.194969, 33.669999)
        (0.200760, 33.630002)
    };
    \addlegendentry{Ours}
    \end{semilogxaxis}%
\end{tikzpicture}%

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/compare_ens_larger.tex <==

\begin{table}[t]
\caption{Larger models. MAE results taken from \citep{assran2022msn}. $^\dagger$ We evaluated the few-shot results using official pretrained weights which are better than the results reported in \cite{assran2022msn}.}
\label{table:compare_ens_merge}
\begin{center}
% \begin{scriptsize}
\small
\adjustbox{max width=\textwidth}{
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Epoch}} &  \multicolumn{4}{c}{\textbf{Few-shot}} & \multicolumn{2}{c}{\textbf{Full-data}} \\
 \cmidrule(lr){3-6}\cmidrule(lr){7-8}
 & & 1 & 2 & 5 & $\sim$13 (1\%) & $k$-NN & Linear \\ 
 \midrule
 \emph{\vitb/16} \\
 \midrule
 iBOT \citep{zhou2022ibot} & 400 & 46.1 $\pm$ 0.3 & 56.2 $\pm$ 0.7  & 64.7 $\pm$ 0.3 & 69.7 & \textbf{77.1} & \textbf{79.5} \\
  MSN \citep{assran2022msn} & 600 & 49.8 $\pm$ 0.2 & 58.9 $\pm$ 0.4 & 65.5 $\pm$ 0.3 & - & - & - \\
%  \multirow{2}{*}{DINO \citep{caron2021dino}} & \vitb/16 & 400 & 41.8 $\pm$ 0.3 & 51.9 $\pm$ 0.6 & 61.4 $\pm$ 0.2 & ? & 76.1 & 78.2 \\  % few-shot result from MSN
DINO$^\dagger$ \citep{caron2021dino}  & 400 & 43.0 $\pm$ 0.2 & 52.7 $\pm$ 0.5 & 61.8 $\pm$ 0.2 & 67.4 & 76.1 & 78.2 \\ % re-evel few-shot result
 \dinop (\retune) & 400 & 49.3 $\pm$ 0.1 & 58.1 $\pm$ 0.5  & 65.0 $\pm$ 0.3  & 69.1 & 76.0 & 78.5 \\ 
 \msnp (\retune) & 400 \\
 \midrule
 \ens[4]{\dinop}{\ew}  & 400 & 51.4 $\pm$ 0.2 & 60.3 $\pm$ 0.6  &  66.7 $\pm$ 0.3 & 70.6 & 76.6 & 79.0 \\
 \ens[16]{\dinop}{\ew} & 400 & \textbf{52.8 $\pm$ 0.1} & \textbf{61.5 $\pm$ 0.4}  &  \textbf{67.6 $\pm$ 0.3} & \textbf{71.1} & \textbf{77.1} & 79.1 \\
 \ens[]{\msnp}{\ew} & 400 \\
 \midrule
%  & \vitb/8 & 300 & 45.8 $\pm$ 0.5 & 55.9 $\pm$ 0.6 & 64.6 $\pm$ 0.2 & 70.0 (?) & 77.4 & 80.1  \\  % few-shot result from MSN
 \emph{\vitb/8} \\
 \midrule
 MSN \citep{assran2022msn} & 600 & 55.1 $\pm$ 0.1 & 64.9 $\pm$ 0.7 & 71.6 $\pm$ 0.3 & - & - & -  \\
DINO$^\dagger$ \citep{caron2021dino} & 300 & 47.5 $\pm$ 0.2 & 57.3 $\pm$ 0.5 & 65.4 $\pm$ 0.3 & 70.3 & 77.4 & 80.1  \\  % re-eval few-shot results
\dinop & 300 & 49.5 $\pm$ 0.5 & 58.6 $\pm$ 0.6  & 65.9 $\pm$ 0.3 & 70.7 & 77.1 & 80.2\\
\msnp (\retune) & 300 \\
\midrule
\ens[4]{\dinop}{\ew} & 300 & 53.8 $\pm$ 0.3 & 62.4 $\pm$ 0.6 & 68.6 $\pm$ 0.4 & 72.6 & 77.9 & 80.7 \\
\ens[16]{\dinop}{\ew} & 300 & \textbf{55.0 $\pm$ 0.4} & \textbf{63.4 $\pm$ 0.6} & \textbf{69.5 $\pm$ 0.3} & \textbf{73.4} & \textbf{78.6} & \textbf{81.0} \\
 \ens[]{\msnp}{\ew} & 300 \\
%  \midrule
%  \emph{\vitl/7} \\
%  \midrule
% MSN \citep{assran2022msn} & 200 & 57.1 $\pm$ 0.6 & 66.4 $\pm$ 0.6 & 72.1 $\pm$ 0.2 & 75.1 & - & 80.7  \\
% \msnp \\
\bottomrule
\end{tabular}
}
% \end{scriptsize}
\end{center}
\vspace{-\baselineskip}
\end{table}


%%%%%%%% OLD: group by method %%%%%%%%
% \begin{table}[h]
% \caption{Larger models. MAE results taken from \citep{assran2022msn}. $^\dagger$ We evaluated the few-shot results using official pretrained weights which are better than the results reported in \cite{assran2022msn}.}
% \label{table:compare_ens_larger}
% \begin{center}
% % \begin{scriptsize}
% \small
% \adjustbox{max width=\textwidth}{
% \begin{tabular}{llccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Arch.}} & \multirow{2}{*}{\textbf{Epoch}} &  \multicolumn{4}{c}{\textbf{Few-shot}} & \multicolumn{2}{c}{\textbf{Full-data}} \\
%  \cmidrule(lr){4-7}\cmidrule(lr){8-9}
%  & & & 1 & 2 & 5 & $\sim$13 (1\%) & $k$-NN & Linear \\ 
%  \midrule
%  \emph{Baseline methods} \\
% %  \midrule
%  \multirow{2}{*}{MAE \citep{he2022mae}} & \vitb/16 & 1600 & 8.2 $\pm$ 0.3 & 25.0 $\pm$ 0.3 & 40.5 $\pm$ 0.2 & - & - & - \\
%  & \vitl/16 & 1600 & 12.3 $\pm$ 0.2 & 19.3 $\pm$ 1.8 & 42.3 $\pm$ 0.3 & - & - & 75.1 \\
%  \multirow{2}{*}{iBOT \citep{zhou2022ibot}} & \vitb/16 & 400 & 46.1 $\pm$ 0.3 & 56.2 $\pm$ 0.7  & 64.7 $\pm$ 0.3 & 69.7 (?) & 77.1 & 79.5 \\
%  & \vitl/16 &  250  & - & - & - & - & 78.0 & 81.0 \\
% %  \midrule
% %  \multirow{2}{*}{DINO \citep{caron2021dino}} & \vitb/16 & 400 & 41.8 $\pm$ 0.3 & 51.9 $\pm$ 0.6 & 61.4 $\pm$ 0.2 & ? & 76.1 & 78.2 \\  % few-shot result from MSN
%   \multirow{2}{*}{DINO$^\dagger$ \citep{caron2021dino}} & \vitb/16 & 400 & 43.0 $\pm$ 0.2 & 52.7 $\pm$ 0.5 & 61.8 $\pm$ 0.2 & 67.4 & 76.1 & 78.2 \\  % re-evel few-shot result
% %  & \vitb/8 & 300 & 45.8 $\pm$ 0.5 & 55.9 $\pm$ 0.6 & 64.6 $\pm$ 0.2 & 70.0 (?) & 77.4 & 80.1  \\  % few-shot result from MSN
%  & \vitb/8 & 300 & 47.5 $\pm$ 0.2 & 57.3 $\pm$ 0.5 & 65.4 $\pm$ 0.3 & 70.3 & 77.4 & 80.1  \\  % re-eval few-shot results
% %  \midrule
%  \dinop (Ours retuned) & \vitb/16 & 400 & 49.3 $\pm$ 0.1 & 58.1 $\pm$ 0.5  & 65.0 $\pm$ 0.3  & 69.1 & 76.0 &  \\ 
%  \multirow{3}{*}{MSN \citep{assran2022msn}} & \vitb/16 & 600 & 49.8 $\pm$ 0.2 & 58.9 $\pm$ 0.4 & 65.5 $\pm$ 0.3 & - & - & - \\
%  & \vitb/8 & 600 & 55.1 $\pm$ 0.1 & 64.9 $\pm$ 0.7 & 71.6 $\pm$ 0.3 & - & - & -  \\
%  & \vitl/7 & 200 & 57.1 $\pm$ 0.6 & 66.4 $\pm$ 0.6 & 72.1 $\pm$ 0.2 & 75.1 & - & 80.7  \\
% \midrule
% \emph{Methods with ensemble heads} \\
%  \ens[4]{\dinop}{\ew} & \vitb/16 & 400 & 51.4 $\pm$ 0.2 & 60.3 $\pm$ 0.6  &  66.7 $\pm$ 0.3 & 70.6 & 76.6 &  \\
%  \ens[16]{\dinop}{\ew} & \vitb/16 & 400 & 52.8 $\pm$ 0.1 & 61.5 $\pm$ 0.4  &  67.6 $\pm$ 0.3 & 71.1 & 77.1 &  \\
% \midrule

% \bottomrule
% \end{tabular}
% }
% % \end{scriptsize}
% \end{center}
% \vspace{-\baselineskip}
% \end{table}

==> tables/compare_ens_s16.tex <==
\begin{table}[t]
\caption{\vits/16, 800 epochs. Note that MSN uses different model to report full-data eval, while we use the same for consistency. Fair comparisons are highlighted in colors.}
\label{table:compare_ens_s16}
\begin{center}
% \begin{scriptsize}
\small
\adjustbox{max width=\textwidth}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Few-shot}} & \multicolumn{2}{c}{\textbf{Full-data}} \\
 \cmidrule(lr){2-5}\cmidrule(lr){6-7}
 & 1 & 2 & 5 & $\sim$13 (1\%) & $k$-NN & Linear \\ 
 \midrule
 \emph{Baseline methods} \\
 \midrule
%  MoCo v3 \citep{chen2021mocov3} &  - & -  &  - & - & - & ~~~-~~ / 73.4\\
 iBOT \citep{zhou2022ibot} & 40.4  $\pm$ 0.5 & 50.8 $\pm$ 0.8  &  59.9 $\pm$ 0.2 & 65.9 & \textbf{75.2} & ~~~-~~ / \textbf{77.9} \\
%  \midrule
DINO \citep{caron2021dino} &  38.9 $\pm$ 0.4 & 48.9 $\pm$ 0.3 & 58.5 $\pm$ 0.1 & 64.5 & 74.5 & 76.1 / 77.0 \\ % few-shot result from MSN
% DINO \citep{caron2021dino} &  38.9 $\pm$ 0.2 & 49.0 $\pm$ 0.2 & 58.5 $\pm$ 0.1 & 64.5 & 74.5 & 76.1 / 77.0 \\  % re-eval few-shot
DINO (\repro) &   39.1 $\pm$ 0.3  &  49.1 $\pm$ 0.5  &  58.6 $\pm$ 0.2  & 64.7 & 74.3 & 75.8 / 76.9 \\
\rowcolor{LightCyan}
\dinop (\retune) &  44.6 $\pm$ 0.2 & 53.6 $\pm$ 0.3   &  61.1 $\pm$ 0.2  & 66.2 & 74.1 & 75.8 / 76.9 \\
% \midrule
% \dinop & 46.2 $\pm$ 0.1   &  54.9 $\pm$ 0.5  &  61.8 $\pm$ 0.5  & 66.6 & 74.0 & 75.8 / 76.8 \\
MSN \citep{assran2022msn} &  47.1 $\pm$ 0.1 & 55.8 $\pm$ 0.6 & 62.8 $\pm$ 0.3 & 67.2 & - & ~~~-~~ / 76.9 \\
% MSN (\repro) &  39.1 $\pm$ 0.3   &  49.2 $\pm$ 0.3  &  58.4 $\pm$ 0.1  & 64.3 & 72.8 & 74.7 / 75.5 \\
% \msnp & 44.0 $\pm$ 0.2   & 52.8 $\pm$ 0.5   &  60.3 $\pm$ 0.1   & 65.0 & 72.7 &  74.6 / 75.9 \\  % 3/1024 head, ME-MAX in MSN setup
% \msnp (Our code; our hyper) &  44.9 $\pm$ 0.2  &  53.7 $\pm$ 0.6 &  60.9 $\pm$ 0.2   &  65.5 & 73.4 & 74.7 / 76.1  \\ % with EMA for codebook
\rowcolor{LightCyan}
\msnp (\retune) &  47.4 $\pm$ 0.1  & 56.3 $\pm$ 0.4  &  62.8 $\pm$ 0.2   &  67.1  & 73.3 &  75.6 / 76.6 \\ % pseudo MSN
\midrule
\emph{Methods with ensemble heads} \\
\midrule
% \ens[4]{\dinop}{\outside}  & 44.2 $\pm$ 0.0  & 53.7 $\pm$ 0.5   & 61.3 $\pm$ 0.3   & 66.2 & 74.2 &  76.0 / 77.0 \\
% \ens[16]{\dinop}{\outside}  & 44.3 $\pm$ 0.3  &  53.3 $\pm$ 0.6  & 61.0 $\pm$ 0.3   & 66.0 & 74.1 &  75.8 / 76.9 \\
% \ens[4]{\dinop}{\inside}  &  44.6 $\pm$ 0.1 &  54.0 $\pm$ 0.5  &   61.8 $\pm$ 0.4 & 66.6 & 74.5 &  76.1 / 77.2 \\
\ens[16]{\dinop}{\inside}  &  45.2 $\pm$ 0.4  &  54.9 $\pm$ 0.4  &  62.5 $\pm$ 0.2  & 67.3 & 75.1 &  76.5 / 77.6 \\
\ens[4]{\dinop}{\ew}  & 46.3 $\pm$ 0.1   &  55.5 $\pm$ 0.6  & 63.0 $\pm$ 0.3   & 67.5 & 74.8 &  76.2 / 77.2 \\
\rowcolor{LightCyan}
\ens[16]{\dinop}{\ew}  &  47.6 $\pm$ 0.1  &  56.8 $\pm$ 0.5  &  64.0 $\pm$ 0.2  & 68.3 & \textbf{75.3} & \textbf{76.8} / \textbf{77.7}  \\
% with EMA for codebook
\ens[2]{\msnp}{\ew}  &  48.8 $\pm$ 0.2  & 57.5 $\pm$ 0.5   &  64.0 $\pm$ 0.2   & 67.9 & 74.6 & 76.0 / 76.9  \\
% \ens[4]{\msnp}{\ew}  &  46.6 $\pm$ 0.2  &  55.3 $\pm$ 0.4  &  62.4 $\pm$ 0.3   & 66.8 & 74.0 & 75.5 / 76.7  \\
\rowcolor{LightCyan}
\ens[8]{\msnp}{\ew}  &  \textbf{50.1 $\pm$ 0.1}  & \textbf{58.9 $\pm$ 0.6}   &  \textbf{65.1 $\pm$ 0.3}   & \textbf{68.7} & \textbf{75.2} & 76.4 / 77.4  \\
% pseudo MSN
\bottomrule
\end{tabular}
}
% \end{scriptsize}
\end{center}
\vspace{-\baselineskip}
\end{table}

==> tables/compare_ens_transfer_b16.tex <==
\begin{table}[h]
\caption{\vitb/16, 400 epochs.}
\label{table:compare_ens_transfer_b16}
\begin{center}
% \begin{scriptsize}
\small
\adjustbox{max width=\textwidth}{
\begin{tabular}{lccccccccc}
\toprule
  & Food101 & CIFAR10 & CIFAR100 & SUN397 & Cars & DTD & Pets & Caltech-101 & Flowers\\
 \midrule
%  DINO & 81.7 & 96.0 & 85.3 & 68.5 & 75.2 &  75.7 & 93.6 & 96.1 & 95.7 \\
 \dinop & 82.2 & 94.8 & 83.6 & 68.8 & 74.2 & 76.9 & 93.0 & 95.7 & 95.9 \\
 \ens[16]{\dinop}{\ew} & 81.9 & 95.0 & 83.6 & 68.5 & 75.7 & 76.0 & 93.8 & 96.1 & 95.3 \\
\bottomrule
\end{tabular}
}
% \end{scriptsize}
\end{center}
\vspace{-\baselineskip}
\end{table}
